Evidence of Galaxy Assembly Bias in SDSS DR7 Galaxy Samples from Count Statistics

We present observational constraints on the galaxy-halo connection, focusing particularly on galaxy assembly bias, from a novel combination of counts-in-cylinders statistics, $P(N_{\rm{CIC}})$, with the standard measurements of the projected two-point correlation function, $w_{\rm{p}}(r_{\rm{p}})$, and number density, $n_{\rm{gal}}$, of galaxies. We measure $n_{\rm{gal}}$, $w_{\rm{p}}(r_{\rm{p}})$ and $P(N_{\rm{CIC}})$ for volume-limited, luminosity-threshold samples of galaxies selected from SDSS DR7, and use them to constrain halo occupation distribution (HOD) models, including a model in which galaxy occupation depends upon a secondary halo property, namely halo concentration. We detect significant positive central assembly bias for the $M_r<-20.0$ and $M_r<-19.5$ samples. Central galaxies preferentially reside within haloes of high concentration at fixed mass. Positive central assembly bias is also favoured in the $M_r<-20.5$ and $M_r<-19.0$ samples. We find no evidence of central assembly bias in the $M_r<-21.0$ sample. We observe only a marginal preference for negative satellite assembly bias in the $M_r<-20.0$ and $M_r<-19.0$ samples, and non-zero satellite assembly bias is not indicated in other samples. Our findings underscore the necessity of accounting for galaxy assembly bias when interpreting galaxy survey data, and demonstrate the potential of count statistics in extracting information from the spatial distribution of galaxies, which could be applied to both galaxy-halo connection studies and cosmological analyses.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

